Reduced Connectivity for Local Bilinear Jacobi Sets

We present a new topological connection method for the local bilinear computation of Jacobi sets that improves the visual representation while preserving the topological structure and geometric configuration. To this end, the topological structure of the local bilinear method is utilized, which is given by the nerve complex of the traditional piecewise linear method. Since the nerve complex consists of higher-dimensional simplices, the local bilinear method (visually represented by the 1-skeleton of the nerve complex) leads to clutter via crossings of line segments. Therefore, we propose a homotopy-equivalent representation that uses different collapses and edge contractions to remove such artifacts. Our new connectivity method is easy to implement, comes with only little overhead, and results in a less cluttered representation.

==> figures/PL_LB_comp.tex <==
\begin{subfigure}[b]{0.4\columnwidth}
	\centering
	\begin{tikzpicture}[font=\small]
	        \coordinate (x1) at (-0.2,0);
			\coordinate (x2) at (1.8,0.1);
			\coordinate (x3) at (0.7,1.3);
			\coordinate (x4) at (1.2,1.1);
			\coordinate (x5) at (-0.5,1.5);
			\coordinate (x6) at (1.25,2.1);
			\coordinate (x7) at (1.8,2.0);
			\coordinate (x8) at (0.8,2.5);
			\coordinate (x9) at (1.8,2.7);
			
			
			%GRID-subsampling
			\coordinate (gs1) at ($ (x1)!0.5!(x2) $);
			\coordinate (gs2) at ($ (x1)!0.5!(x3) $);
			\coordinate (gs3) at ($ (x3)!0.5!(x2) $); %%
			\coordinate (gs4) at ($ (x1)!0.5!(x5) $);
			\coordinate (gs5) at ($ (x5)!0.5!(x3) $);
			\coordinate (gs6) at ($ (x5)!0.5!(x6) $);
			\coordinate (gs7) at ($ (x3)!0.5!(x6) $);
			\coordinate (gs8) at ($ (x5)!0.5!(x8) $);
			\coordinate (gs9) at ($ (x6)!0.5!(x8) $);
			\coordinate (gs10) at ($ (x3)!0.5!(x4) $); %%
			\coordinate (gs11) at ($ (x4)!0.5!(x6) $); %%
			\coordinate (gs12) at ($ (x6)!0.5!(x9) $); %%
			\coordinate (gs13) at ($ (x9)!0.5!(x8) $);
			
			
			%Divide edges
			\coordinate (je1) at  ($ (x1)!0.5!(x3) $);
			\coordinate (je2) at  ($ (x3)!0.5!(x6) $);
			\coordinate (je3) at  ($ (x6)!0.5!(x8) $);
			
			\coordinate (je4) at  ($ (x1)!0.5!(gs2) $);
			\coordinate (je5) at  ($ (gs2)!0.5!(gs5) $);
			\coordinate (je6) at  ($ (gs5)!0.5!(gs7) $);
			\coordinate (je7) at  ($ (gs7)!0.5!(gs6) $);
			\coordinate (je8) at  ($ (gs6)!0.5!(gs8) $);
			
			%JACOBISET Points
			\coordinate (jh1) at  ($ (x1)!0.4!(x2) $);
			
			\coordinate (jp1) at ($ (x5)!0.75!(je1) $);
			\coordinate (jp2) at ($ (x5)!0.7!(je2) $);
			\coordinate (jp3) at ($ (x5)!0.8!(je3) $);
			\coordinate (jh2) at  ($ (x5)!0.7!(x8) $);
	
			%\fill[blue]	(jp1)	circle [radius = 1pt];
			%\fill[blue]	(jp2)	circle [radius = 1pt];
			%\fill[blue]	(jp3)	circle [radius = 1pt];
			
			\draw [-,thin]  %DRAW TRIANGULATION
			(x1) -- (x2)
			%(x1) -- (x3)
			(x2) -- (x3)
			(x2) -- (x4)
			(x1) -- (x5)
			(x3) -- (x4)
			(x3) -- (x5)
			%(x3) -- (x6)
			(x5) -- (x6)
			(x6) -- (x7)
			(x6) -- (x4)
			(x7) -- (x4)
			(x5) -- (x8)
			%(x6) -- (x8)
			(x6) -- (x9)
			(x7) -- (x9)
			(x8) -- (x9);
			
			\draw [-, red, thick] (x1) -- (x3) -- (x6) -- (x8); %DRAW Edelsbrunner JS
			
			\fill[black]	(x1)	circle [radius = 2pt];
			\fill[black]	(x2)	circle [radius = 2pt];
			\fill[black]	(x3)	circle [radius = 2pt];
			\fill[black]	(x4)	circle [radius = 2pt];
			\fill[black]	(x5)	circle [radius = 2pt];
			\fill[black]	(x6)	circle [radius = 2pt];
			\fill[black]	(x7)	circle [radius = 2pt];
			\fill[black]	(x8)	circle [radius = 2pt];
			\fill[black]	(x9)	circle [radius = 2pt];
			
			%\draw[-, blue, thick] (jh1) -- (jp1) -- (jp2) -- (jp3) -- (jh2);
			\draw[densely dotted, purple] (x5) -- (je1) -- (x2);
			\draw[densely dotted, purple] (x4) -- (je2)--(x5);
			\draw[densely dotted, purple] (x5) -- (je3) -- (x9);
			
			\draw (x1) node [left] 			{${\vec{x}_1}$}
			(x2) node [right] 			{${\vec{x}_2}$}
			(x3) node [below right] 			{${\vec{x}_3}$}
			(x4) node [right] 			{${\vec{x}_4}$}
			(x5) node [left] 			{${\vec{x}_5}$}
			(x6) node [below right] 			{${\vec{x}_6}$}
			(x7) node [right] 			{${\vec{x}_7}$}
			(x8) node [left] 			{${\vec{x}_8}$}
			(x9) node [right] 			{${\vec{x}_9}$};
	\end{tikzpicture}
	\caption{Criticality of edges}
	\label{fig:method_PL}
\end{subfigure}
\begin{subfigure}[b]{0.4\columnwidth}
	\centering
	\begin{tikzpicture}[font=\small]
	
			\fill[blue]	(jp1)	circle [radius = 1pt];
			\fill[blue]	(jp2)	circle [radius = 1pt];
			\fill[blue]	(jp3)	circle [radius = 1pt];
			
			\draw [-,thin]  %DRAW TRIANGULATION
			(x1) -- (x2)
			%(x1) -- (x3)
			(x2) -- (x3)
			(x2) -- (x4)
			(x1) -- (x5)
			(x3) -- (x4)
			(x3) -- (x5)
			%(x3) -- (x6)
			(x5) -- (x6)
			(x6) -- (x7)
			(x6) -- (x4)
			(x7) -- (x4)
			(x5) -- (x8)
			%(x6) -- (x8)
			(x6) -- (x9)
			(x7) -- (x9)
			(x8) -- (x9);
			
			\draw [-, red, thick] (x1) -- (x3) -- (x6) -- (x8); %DRAW Edelsbrunner JS
			
			\fill[black]	(x1)	circle [radius = 2pt];
			\fill[black]	(x2)	circle [radius = 2pt];
			\fill[black]	(x3)	circle [radius = 2pt];
			\fill[black]	(x4)	circle [radius = 2pt];
			\fill[black]	(x5)	circle [radius = 2pt];
			\fill[black]	(x6)	circle [radius = 2pt];
			\fill[black]	(x7)	circle [radius = 2pt];
			\fill[black]	(x8)	circle [radius = 2pt];
			\fill[black]	(x9)	circle [radius = 2pt];
			
			\draw[densely dotted, purple] (x5) -- (je1) -- (x2);
			\draw[densely dotted, purple] (x4) -- (je2)--(x5);
			\draw[densely dotted, purple] (x5) -- (je3) -- (x9);
			%\draw[-, blue, thick] (jh1) -- (jp1) -- (jp2) -- (jp3) -- (jh2);
			
			\draw (x1) node [left] 			{${\vec{x}_1}$}
			(x2) node [right] 			{${\vec{x}_2}$}
			(x3) node [below right] 			{${\vec{x}_3}$}
			(x4) node [right] 			{${\vec{x}_4}$}
			(x5) node [left] 			{${\vec{x}_5}$}
			(x6) node [below right] 			{${\vec{x}_6}$}
			(x7) node [right] 			{${\vec{x}_7}$}
			(x8) node [left] 			{${\vec{x}_8}$}
			(x9) node [right] 			{${\vec{x}_9}$};
	\end{tikzpicture}
	\caption{Mark Jacobi set points}
	\label{fig:method_JSP}
\end{subfigure}
\begin{subfigure}[b]{0.4\columnwidth}
	\centering
	\begin{tikzpicture}[font=\small]
		
			\fill[blue]	(jp1)	circle [radius = 1pt];
			\fill[blue]	(jp2)	circle [radius = 1pt];
			\fill[blue]	(jp3)	circle [radius = 1pt];
			
			\draw [-,thin]  %DRAW TRIANGULATION
			(x1) -- (x2)
			%(x1) -- (x3)
			(x2) -- (x3)
			(x2) -- (x4)
			(x1) -- (x5)
			(x3) -- (x4)
			(x3) -- (x5)
			%(x3) -- (x6)
			(x5) -- (x6)
			(x6) -- (x7)
			(x6) -- (x4)
			(x7) -- (x4)
			(x5) -- (x8)
			%(x6) -- (x8)
			(x6) -- (x9)
			(x7) -- (x9)
			(x8) -- (x9);
			
			\draw [-, red, thick] (x1) -- (x3) -- (x6) -- (x8); %DRAW Edelsbrunner JS
			
			\fill[black]	(x1)	circle [radius = 2pt];
			\fill[black]	(x2)	circle [radius = 2pt];
			\fill[black]	(x3)	circle [radius = 2pt];
			\fill[black]	(x4)	circle [radius = 2pt];
			\fill[black]	(x5)	circle [radius = 2pt];
			\fill[black]	(x6)	circle [radius = 2pt];
			\fill[black]	(x7)	circle [radius = 2pt];
			\fill[black]	(x8)	circle [radius = 2pt];
			\fill[black]	(x9)	circle [radius = 2pt];
			
			\draw[-, blue, thick] (jh1) -- (jp1) -- (jp2) -- (jp3) -- (jh2);
			
			\draw (x1) node [left] 			{${\vec{x}_1}$}
			(x2) node [right] 			{${\vec{x}_2}$}
			(x3) node [below right] 			{${\vec{x}_3}$}
			(x4) node [right] 			{${\vec{x}_4}$}
			(x5) node [left] 			{${\vec{x}_5}$}
			(x6) node [below right] 			{${\vec{x}_6}$}
			(x7) node [right] 			{${\vec{x}_7}$}
			(x8) node [left] 			{${\vec{x}_8}$}
			(x9) node [right] 			{${\vec{x}_9}$};
	\end{tikzpicture}
	\caption{Connect Jacobi set points}\label{fig:our_approach}
	\label{fig:method_CJS}
\end{subfigure}

==> sections/sec-notes.tex <==
\onecolumn

\vspace{0.5cm}
{\Large Notes:}\\

\vspace{0.5cm}
{\large Individual Todos and tasks:}
\vspace{0.5cm}
\begin{itemize}
	\setlength\itemsep{0em}
	\item @ \textbf{Bei} and \textbf{Ingrid}: Related Works (again) with focus on Simplicial Collapses (if you are busy, please insert / copy paste titles of relevant papers, so we can write it) and maybe brief idea of what to introduce in the Background chapter
	\item @ \textbf{Youjia}: Find new examples for presentation and Comparison of Jacobi Sets 
	\item @ \textbf{Tim and Daniel K.}: 
	\begin{itemize}
	    \item Write down and implementation!
	\end{itemize}
\end{itemize}

\vspace{0.5cm}
TODO
\begin{itemize}
    \item check if double blinded or not ??? Now single-blind review process. That's clear.
    \item Spelling to check for consistency:
\begin{itemize}
	\setlength\itemsep{0em}
	\item $\{a,v_1, b,v_2\}$-cell
	\item Multi-field
	\item scalar field
	\item Cylinder Flow with a von Kármán vortex street
	\item real world dataset
	\item line segment
	\item Hurricane Isabel dataset
	\item 3D / 2D
	\item Algorithm 1, Figure 1 , ...
	\item higher-dimensional ...
\end{itemize}
\end{itemize}
\vspace{0.5cm}
IDEAS:
\begin{itemize}
    \item One can see our method as extension of the local bilinear method, especially the Algorithm 2, the connection of Jacobi set points.
    \item Our method doesn't introduce much computational overhead -> evaluation
    \item Discribe more clearly where the analogy of 1-dimensional manifolds come from (folding - unfolding)
    \item Compare Number of edges for different datasets.
\end{itemize}


\newpage

\twocolumn

